NeX: Real-time View Synthesis with Neural Basis Expansion

We present NeX, a new approach to novel view synthesis based on enhancements of multiplane image (MPI) that can reproduce next-level view-dependent effects -- in real time. Unlike traditional MPI that uses a set of simple RGB$\alpha$ planes, our technique models view-dependent effects by instead parameterizing each pixel as a linear combination of basis functions learned from a neural network. Moreover, we propose a hybrid implicit-explicit modeling strategy that improves upon fine detail and produces state-of-the-art results. Our method is evaluated on benchmark forward-facing datasets as well as our newly-introduced dataset designed to test the limit of view-dependent modeling with significantly more challenging effects such as rainbow reflections on a CD. Our method achieves the best overall scores across all major metrics on these datasets with more than 1000$\times$ faster rendering time than the state of the art. For real-time demos, visit https://nex-mpi.github.io/

==> content/4_failure_case.tex <==
% picture contain failure case from labjuice and food


\begin{figure}
    \centering
    \setlength\tabcolsep{1.5pt}
    \begin{tabular}{cccc}
        \begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/food/crop/000_gt.png}\end{subfigure}
        & \begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/food/crop/000_ours.png}\end{subfigure} 
        & \begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/labjuice/crop/000_gt.png}\end{subfigure}
        & \begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/labjuice/crop/000_ours.png}\end{subfigure} \\
        Ground truth & \textbf{Ours} & Ground truth & \textbf{Ours}
    
    \end{tabular}
    %\begin{tabular}{cc}
    %    \shortstack{ 
    %      \begin{overpic}[width=0.4\linewidth]{./images/result/food/000_gt.png}
    %         \put(3,3){\includegraphics[width=1.5cm,frame]{./images/result/food/crop/000_gt.png}}  
    %      \end{overpic} }
    %    & \shortstack{ 
    %      \begin{overpic}[width=0.4\linewidth]{./images/result/food/000_ours.png}
    %         \put(3,3){\includegraphics[width=1.5cm,frame]{./images/result/food/crop/000_ours.png}}  
    %      \end{overpic} }
    %    \\
    %    \shortstack{ 
    %      \begin{overpic}[width=0.4\linewidth]{./images/result/labjuice/000_gt.png}
    %         \put(3,3){\includegraphics[width=1.5cm,frame]{./images/result/labjuice/crop/000_gt.png}}  
    %      \end{overpic}
    %     \\  Ground truth}
    %    & \shortstack{ 
    %      \begin{overpic}[width=0.4\linewidth]{./images/result/labjuice/000_ours.png}
    %         \put(3,3){\includegraphics[width=1.5cm,frame]{./images/result/labjuice/crop/000_ours.png}}  
    %      \end{overpic}
    %     \\ NeX (Ours)}
    %\end{tabular}
    \caption{Our failure cases on a crystal candle holder in scene Food (Left) and test tubes in scene Lab (Right).}
    \label{fig_failure_}
\end{figure}

% Our failure cases include the lack of sharp sparkles in the crystal candle holder in scene Food and the reflection of tube rack in scene Lab which shown in figure

==> content/4figure2.tex <==

\begin{figure}
    \centering
    \setlength\tabcolsep{1.5pt}
    \begin{tabular}{ccc}
    \multicolumn{3}{c}{ \includegraphics[width=6cm]{./images/result/space056/cam05_ours.png} }\\
        \shortstack{ 
          \includegraphics[width=0.11\textwidth]{./images/result/space056/crop1/org.png}
         \\ Ground truth}
        & \shortstack{ 
          \includegraphics[width=0.11\textwidth]{./images/result/space056/crop1/our.png}
         \\ NeX (Ours)}
        & \shortstack{
          \includegraphics[width=0.11\textwidth]{./images/result/space056/crop1/deepv.png}
         \\ DeepView\cite{flynn2019deepview} }

    \end{tabular}
    \caption{Our synthesized results on the DeepView\cite{flynn2019deepview}'s Space dataset. (\textbf{Top}) The results is synthesized from 12 input views. (\textbf{Bottom}) we show a zooming crop version of ground truth(left), Our NeX (center), and DeepView (right).}
    \label{fig_DeepView}
\end{figure}



==> content/4figure3.tex <==
\begin{figure*}
    \label{fig-nerfvisual}
    \centering
    \renewcommand{\arraystretch}{3}
    \setlength\tabcolsep{1.5pt}
    \renewcommand{\arraystretch}{1}
    \begin{tabular}{cccccccc}
        
        \multirow{2}{*}[2em]{
                \shortstack{\includegraphics[width=3cm]{./images/result/pasta/000_gt.png} 
                \\ Orchids}} 
        & \begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/pasta/crop/org.png}\end{subfigure}
        & \begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/pasta/crop/our.png}\end{subfigure}
        & \begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/pasta/crop/nerf.png}\end{subfigure} 
        \bigstrut 
        &
        \multirow{2}{*}[2em]{
                \shortstack{\includegraphics[width=3cm]{./images/result/crest/008_ours.png} 
                \\ Leaves}} 
        & \begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/crest/crop1/org.png}\end{subfigure}
        & \begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/crest/crop1/our.png}\end{subfigure}
        & \begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/crest/crop1/nerf.png}\end{subfigure} 
        \bigstrut \\
        & \shortstack{\begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/leaves/crop2/org_s.png}\end{subfigure}
            \\ Ground truth}
        & \shortstack{\begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/leaves/crop2/our_s.png}\end{subfigure}
            \\ NeX (Ours) }
        & \shortstack{\begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/leaves/crop2/nerf_s.png}\end{subfigure} 
            \\ NeRF\cite{mildenhall2020nerf}}
        \bigstrut 
        &
        & \shortstack{\begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/crest/crop2/org.png}\end{subfigure}
            \\ Ground truth}
        & \shortstack{\begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/crest/crop2/our.png}\end{subfigure}
            \\ NeX (Ours) }
        & \shortstack{\begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/crest/crop2/nerf.png}\end{subfigure} 
            \\ NeRF\cite{mildenhall2020nerf}}
        \bigstrut \\
    \end{tabular}
    \caption{
    Qualitatively comparions on Shiny dataset between ground truth, Our NeX , and NeRF\cite{mildenhall2020nerf}.
    }
\end{figure*}

==> content/4figure4.tex <==
\begin{figure*}
    \centering
    \setlength\tabcolsep{1.5pt}
    \begin{tabular}{ccc}
        \shortstack{ 
          \begin{overpic}[width=5.0cm]{./images/result/crest/008_gt.png}
             \put(3,3){\includegraphics[width=1.5cm,frame]{./images/result/crest/crop1/org.png}}  
          \end{overpic}
         \\ Ground truth}
        & \shortstack{ 
          \begin{overpic}[width=5.0cm]{./images/result/crest/008_ours.png}
             \put(3,3){\includegraphics[width=1.5cm,frame]{./images/result/crest/crop1/our.png}}  
          \end{overpic}
         \\ NeX (Ours)}
        & \shortstack{
          \begin{overpic}[width=5.0cm]{./images/result/crest/008_nerf.png}
             \put(3,3){ \includegraphics[width=1.5cm,frame]{./images/result/crest/crop1/nerf.png}}  
          \end{overpic}
         \\ NeRF }
    \end{tabular}
    \caption{qualitatively comparions on Shiny dataset between ground truth(left), Our NeX (center), and NeRF\cite{mildenhall2020nerf} (right).}
    \label{fig_shiny}
\end{figure*}

==> content/4figure_new_opt.tex <==

\begin{figure}
    \centering
    \setlength\tabcolsep{1.5pt}
    \begin{tabular}{ccc}
    \multicolumn{3}{c}{ \includegraphics[width=6cm]{./images/result/optical_comparison/112_ours.png} }\\
        \shortstack{ 
          \includegraphics[width=0.11\textwidth]{./images/result/optical_comparison/1/crop_112_gt_1.png}
         \\ Ground Truth}
        & \shortstack{ 
          \includegraphics[width=0.11\textwidth]{./images/result/optical_comparison/1/crop_112_ours_1.png}
         \\ \texbf{Ours}}
        & \shortstack{
          \includegraphics[width=0.11\textwidth]{./images/result/optical_comparison/1/crop_112_nerf_1.png}
         \\ NeRF\cite{mildenhall2020nerf} }
    \bigstrut \\
    \addlinespace
    \multicolumn{3}{c}{ \includegraphics[width=6cm]{./images/result/wrench_comparison/000_ours.png} }\\
        \shortstack{ 
          \includegraphics[width=0.11\textwidth]{./images/result/wrench_comparison/0/crop_000_gt_0.png}
         \\ Ground truth}
        & \shortstack{ 
          \includegraphics[width=0.11\textwidth]{./images/result/wrench_comparison/0/crop_000_ours_0.png}
         \\ \texbf{Ours}}
        & \shortstack{
          \includegraphics[width=0.11\textwidth]{./images/result/wrench_comparison/0/crop_000_nerf_0.png}
         \\ NeRF\cite{mildenhall2020nerf} }
    \end{tabular}
    \caption{Qualitative results on test views from challenging shiny dataset. Our method can bring some part of the reflection lined air vent back and spiral coils, while NeRF performs blurrier. We urge readers to see our website for apparent differences. }
    \label{fig_deepview}
\end{figure}



==> content/4figure_optical_com.tex <==

    
\begin{figure*}
    \label{fig-shinyvisual}
    \renewcommand{\arraystretch}{3}
    \setlength\tabcolsep{1.5pt}
    \renewcommand{\arraystretch}{1}
    \begin{tabular}{cccc}
        
        \multirow{2}{*}[4em]{
                \shortstack{\includegraphics[width=3cm]{./images/result/optical_comparison/112_gt.png} 
                \\ CD}} 
        & \begin{subfigure}[b]{0.08\textwidth}\includegraphics[width=\textwidth]{./images/result/optical_comparison/0/crop_112_gt_0.png}\end{subfigure}
        & \begin{subfigure}[b]{0.08\textwidth}\includegraphics[width=\textwidth]{./images/result/optical_comparison/0/crop_112_ours_0.png}\end{subfigure}
        & \begin{subfigure}[b]{0.08\textwidth}\includegraphics[width=\textwidth]{./images/result/optical_comparison/0/crop_112_nerf_0.png}\end{subfigure} 
        \bigstrut \\
        & \begin{subfigure}[b]{0.08\textwidth}\includegraphics[width=\textwidth]{./images/result/optical_comparison/1/crop_112_gt_1.png}\end{subfigure}
        & \begin{subfigure}[b]{0.08\textwidth}\includegraphics[width=\textwidth]{./images/result/optical_comparison/1/crop_112_ours_1.png}\end{subfigure}
        & \begin{subfigure}[b]{0.08\textwidth}\includegraphics[width=\textwidth]{./images/result/optical_comparison/1/crop_112_nerf_1.png}\end{subfigure} 
        \bigstrut \\
        \addlinespace
        \multirow{2}{*}[4em]{
                \shortstack{\includegraphics[width=3cm]{./images/result/wrench_comparison/000_gt.png} 
                \\ Tools}} 
        & \begin{subfigure}[b]{0.08\textwidth}\includegraphics[width=\textwidth]{./images/result/wrench_comparison/0/crop_000_gt_0.png}\end{subfigure}
        & \begin{subfigure}[b]{0.08\textwidth}\includegraphics[width=\textwidth]{./images/result/wrench_comparison/0/crop_000_ours_0.png}\end{subfigure}
        & \begin{subfigure}[b]{0.08\textwidth}\includegraphics[width=\textwidth]{./images/result/wrench_comparison/0/crop_000_nerf_0.png}\end{subfigure} 
        \bigstrut \\
        & \shortstack{\begin{subfigure}[b]{0.08\textwidth}\includegraphics[width=\textwidth]{./images/result/wrench_comparison/1/crop_000_gt_1.png}\end{subfigure}
            \\ Ground Truth}
        & \shortstack{\begin{subfigure}[b]{0.08\textwidth}\includegraphics[width=\textwidth]{./images/result/wrench_comparison/1/crop_000_ours_1.png}\end{subfigure}
            \\ NeX (Ours) }
        & \shortstack{\begin{subfigure}[b]{0.08\textwidth}\includegraphics[width=\textwidth]{./images/result/wrench_comparison/1/crop_000_nerf_1.png}\end{subfigure} 
            \\ NeRF\cite{mildenhall2020nerf}}
        \bigstrut \\
    \end{tabular}
    \caption{
    Qualitative results on test views from challenging shiny dataset. In CD scene, our method can bring some part of lined air vent back, while NeRF fail to capture. 
    }
\end{figure*}

==> content/RecycleBin/4figure.tex <==


%\begin{figure*}
%        \begin{tabular}{c|c}
%            \multirow{2}{*}{ 
%                    \thead{ \includegraphics[width=0.25\textwidth]{./images/result/fern/fern016_gt.png} ..\\ fern } }
%            & %\multicolumn{2}{l}
%            { \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/fern/crop1/our.png}\end{subfigure} }
%            { \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/fern/crop1/nerf.png}\end{subfigure} }
%            { \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/fern/crop1/llff.png}\end{subfigure} } \\
%            & %\multicolumn{1}{l} 
%            { \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/fern/crop2/our.png}\end{subfigure} }
%            { \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/fern/crop2/nerf.png}\end{subfigure} }
%            { \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/fern/crop2/llff.png}\end{subfigure} } \\
%            
%            \multirow{2}{*}{
%                    \includegraphics[width=0.25\textwidth]{./images/result/leaves/leaves000_gt.png} 
%                    %\caption{leaves}
%                    }
%            & %\multicolumn{1}{l}
%            { \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/leaves/crop1/our.png}\end{subfigure} }
%            { \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/leaves/crop1/nerf.png}\end{subfigure} }
%            { \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/leaves/crop1/llff.png}\end{subfigure} } \\
%            & %\multicolumn{1}{l}
%            { \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/leaves/crop2/our.png}\end{subfigure} }
%            { \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/leaves/crop2/nerf.png}\end{subfigure} }
%            { \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/leaves/crop2/llff.png}\end{subfigure} } \\
%            %\ttfamily xxx & \ttfamily xxx & \ttfamily xxx \\                \hline
%        \end{tabular}
%\end{figure*}


%\renewcommand{\multirowsetup}{\centering}
%\begin{tabular}{c|c}
%\multirow{2}[2]{*}[2mm]{\begin{subfigure}[b]{0.25\textwidth}\includegraphics[width=\textwidth]{./images/result/fern/fern016_gt.png}\end{subfigure} } 
%fern & \includegraphics[width=0.15\textwidth]{./images/result/fern/crop1/our.png} \\
%& \includegraphics[width=0.15\textwidth]{./images/result/fern/crop2/our.png}
%\end{tabular}

%\begin{table}
%\centering
%\renewcommand{\arraystretch}{3}
%\begin{tabular}{ccc}
%    \toprule
%    Sections & Axis & Imperfections\\
%    \midrule
%    \multirow{2}[2]{*}[2mm]{\includegraphics[width=3cm]{./images/result/fern/fern016_gt.png}} & $y-y$ & $\dfrac{L}{200}$ \bigstrut \\
%                                                                              & $z-z$ & $\dfrac{L}{150}$ \bigstrut \\
%    \bottomrule
%\end{tabular}
%\end{table}

\begin{figure*}
    \label{fig-nerfvisual}
    \centering
    \renewcommand{\arraystretch}{3}
    \setlength\tabcolsep{1.5pt}
    \renewcommand{\arraystretch}{1}
    \begin{tabular}{ccccc}
        \multirow{2}[2]{*}[2mm]{
                \shortstack{\includegraphics[width=4cm]{./images/result/fern/fern016_gt.png} 
                \\ Fern}} 
        & \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/fern/crop1/org.png}\end{subfigure}
        & \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/fern/crop1/our.png}\end{subfigure}
        & \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/fern/crop1/nerf.png}\end{subfigure} 
        & \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/fern/crop1/llff.png}\end{subfigure}
        \bigstrut \\
        & \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/fern/crop2/org.png}\end{subfigure}
        & \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/fern/crop2/our.png}\end{subfigure}
        & \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/fern/crop2/nerf.png}\end{subfigure} 
        & \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/fern/crop2/llff.png}\end{subfigure}
        \bigstrut \\
        
        \multirow{2}[2]{*}[2mm]{
                \shortstack{\includegraphics[width=4cm]{./images/result/orchids/orchid000_gt.png} 
                \\ Orchids}} 
        & \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/orchids/crop1/org.png}\end{subfigure}
        & \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/orchids/crop1/our.png}\end{subfigure}
        & \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/orchids/crop1/nerf.png}\end{subfigure} 
        & \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/orchids/crop1/llff.png}\end{subfigure}
        \bigstrut \\
        & \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/orchids/crop2/org.png}\end{subfigure}
        & \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/orchids/crop2/our.png}\end{subfigure}
        & \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/orchids/crop2/nerf.png}\end{subfigure} 
        & \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/orchids/crop2/llff.png}\end{subfigure}
        \bigstrut \\
        
        \multirow{2}[2]{*}[2mm]{
                \shortstack{\includegraphics[width=4cm]{./images/result/leaves/leaves000_gt.png} 
                \\ Leaves}} 
        & \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/leaves/crop1/org.png}\end{subfigure}
        & \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/leaves/crop1/our.png}\end{subfigure}
        & \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/leaves/crop1/nerf.png}\end{subfigure} 
        & \begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/leaves/crop1/llff.png}\end{subfigure}
        \bigstrut \\
        & \shortstack{\begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/leaves/crop2/org.png}\end{subfigure}
            \\ Ground Truth}
        & \shortstack{\begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/leaves/crop2/our.png}\end{subfigure}
            \\ Ours}
        & \shortstack{\begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/leaves/crop2/nerf.png}\end{subfigure} 
            \\ NeRF\cite{mildenhall2020nerf}}
        & \shortstack{\begin{subfigure}[b]{0.15\textwidth}\includegraphics[width=\textwidth]{./images/result/leaves/crop2/llff.png}\end{subfigure}
            \\ LLFF\cite{mildenhall2019local} }
        \bigstrut \\
    \end{tabular}
    \caption{
    Results on test views from NeRF's real forward-facing dataset. Our method captures more complete geometry than LLFF and SRN as can be seen in Orchids scene and recovers fine detail better than all other methods seen in Leaves scene.
    %Comparisons on test-set views of NeRF's real forward-facing dataset.
    %NeRF has more complete geometry than LLFF, as shown in Orchid's petals. 
    %In the other hand, LLFF, which based on MPI, is better in very fine detail texture, as shown in Leaves' crop.
    %Our method is able to well represent both fine detail and geometry. 
    }
\end{figure*}

==> content/RecycleBin/4figure2.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}[b]{0.15\textwidth}
      \centering
       \includegraphics[width=\textwidth]{./images/result/fern/crop1/org.png}
  \end{subfigure}
  \hfill
   \begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\textwidth]{./images/result/fern/crop1/our.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\textwidth]{./images/result/fern/crop1/nerf.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\textwidth]{./images/result/fern/crop1/llff.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\textwidth]{./images/result/fern/crop1/srn.png}
  \end{subfigure}
  
  %\newline
  
    \begin{subfigure}[b]{0.15\textwidth}
      \centering
       \includegraphics[width=\textwidth]{./images/result/fern/crop2/org.png}
  \end{subfigure}
  \hfill
   \begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\textwidth]{./images/result/fern/crop2/our.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\textwidth]{./images/result/fern/crop2/nerf.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\textwidth]{./images/result/fern/crop2/llff.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\textwidth]{./images/result/fern/crop2/srn.png}
  \end{subfigure}
  
   % \newline
    
  \begin{subfigure}[b]{0.15\textwidth}
   \centering
   \includegraphics[width=\textwidth]{./images/result/orchids/crop1/org.png}
  \end{subfigure}
  \hfill
   \begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\textwidth]{./images/result/orchids/crop1/our.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\textwidth]{./images/result/orchids/crop1/nerf.png}
  \end{subfigure}
  \hfill
   \begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\textwidth]{./images/result/orchids/crop1/llff.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\textwidth]{./images/result/orchids/crop1/srn.png}
  \end{subfigure}
  
     % \newline
    
  \begin{subfigure}[b]{0.15\textwidth}
   \centering
   \includegraphics[width=\textwidth]{./images/result/orchids/crop2/org.png}
  \end{subfigure}
  \hfill
   \begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\textwidth]{./images/result/orchids/crop2/our.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\textwidth]{./images/result/orchids/crop2/nerf.png}
  \end{subfigure}
  \hfill
   \begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\textwidth]{./images/result/orchids/crop2/llff.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\textwidth]{./images/result/orchids/crop2/srn.png}
  \end{subfigure}
  
   % \newline
    
  \begin{subfigure}[b]{0.15\textwidth}
   \centering
   \includegraphics[width=\textwidth]{./images/result/leaves/crop1/org.png}
  \end{subfigure}
  \hfill
   \begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\textwidth]{./images/result/leaves/crop1/our.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\textwidth]{./images/result/leaves/crop1/nerf.png}
  \end{subfigure}
  \hfill
   \begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\textwidth]{./images/result/leaves/crop1/llff.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\textwidth]{./images/result/leaves/crop1/srn.png}
  \end{subfigure}
  
  
    %  \newline
    
  \begin{subfigure}[b]{0.15\textwidth}
   \centering
   \includegraphics[width=\textwidth]{./images/result/leaves/crop2/org.png}
      \caption{Ground Truth}
  \end{subfigure}
  \hfill
   \begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\textwidth]{./images/result/leaves/crop2/our.png}
    \caption{Our}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\textwidth]{./images/result/leaves/crop2/nerf.png}
    \caption{NeRF \cite{mildenhall2020nerf}}
  \end{subfigure}
  \hfill
   \begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\textwidth]{./images/result/leaves/crop2/llff.png}
    \caption{LLFF \cite{mildenhall2019local}}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\textwidth]{./images/result/leaves/crop2/srn.png}
    \caption{SRN \cite{sitzmann2019srns}}
  \end{subfigure}
  \caption{Comparison our model in different components. }
  \label{fig-comparedegree}
\end{figure*}


==> content/RecycleBin/4figure3.tex <==
\begin{figure*}
    \centering
    \label{fig-nerfvisual}
    \setlength\tabcolsep{1.5pt}
    \begin{tabular}{ccccCCCC}
    \multicolumn{4}{c}{ \includegraphics[width=7cm]{./images/result/fern/fern_our.png} }
    &
    \multicolumn{4}{c}{ \includegraphics[width=7cm]{./images/result/orchids/orchid_our.png} }\\
        \shortstack{ 
          \includegraphics[width=0.10\textwidth]{./images/result/fern/crop1/org.png}
           }
        & \shortstack{ 
          \includegraphics[width=0.10\textwidth]{./images/result/fern/crop1/our.png}
           }
        & \shortstack{
          \includegraphics[width=0.10\textwidth]{./images/result/fern/crop1/nerf.png}
          }
        & \shortstack{
          \includegraphics[width=0.10\textwidth]{./images/result/fern/crop1/llff.png}
          }
        &
        \shortstack{ 
          \includegraphics[width=0.10\textwidth]{./images/result/orchids/crop1/org.png}
           }
        & \shortstack{ 
          \includegraphics[width=0.10\textwidth]{./images/result/orchids/crop1/our.png}
           }
        & \shortstack{
          \includegraphics[width=0.10\textwidth]{./images/result/orchids/crop1/nerf.png}
          }
        & \shortstack{
          \includegraphics[width=0.10\textwidth]{./images/result/orchids/crop1/llff.png}
          }
     \\
        \shortstack{ 
          \includegraphics[width=0.10\textwidth]{./images/result/fern/crop2/org.png}\\
          Ground truth
           }
        & \shortstack{ 
          \includegraphics[width=0.10\textwidth]{./images/result/fern/crop2/our.png}\\
          Ours
           }
        & \shortstack{
          \includegraphics[width=0.10\textwidth]{./images/result/fern/crop2/nerf.png}\\
          NeRF \cite{mildenhall2020nerf}
          }
        & \shortstack{
          \includegraphics[width=0.10\textwidth]{./images/result/fern/crop2/llff.png}\\
          LLFF \cite{mildenhall2019local}
          }
        &
        \shortstack{ 
          \includegraphics[width=0.10\textwidth]{./images/result/orchids/crop2/org.png}\\
          Ground truth
           }
        & \shortstack{ 
          \includegraphics[width=0.10\textwidth]{./images/result/orchids/crop2/our.png}\\
          Ours
           }
        & \shortstack{
          \includegraphics[width=0.10\textwidth]{./images/result/orchids/crop2/nerf.png}\\
          NeRF \cite{mildenhall2020nerf}
          }
        & \shortstack{
          \includegraphics[width=0.10\textwidth]{./images/result/orchids/crop2/llff.png}\\
          LLFF \cite{mildenhall2019local}
          }
    \end{tabular}
    
    \caption{Results on test views from NeRF's real forward-facing dataset. Our method captures more complete geometry than LLFF and SRN as can be seen in Orchids scene and recovers fine detail better than all other methods shown in Leaves scene.
    %and reconstruct more and  NeRF has more complete geometry than LLFF, as shown in Orchid's petals. On the other hand, MPI-based LLFF captures finer detail, as shown in Leaves' crop.
    %Our method is able to well represent both fine detail and geometry. 
    }
\end{figure*}

==> content/RecycleBin/4figure4.tex <==
\begin{figure*}
    \centering
    \renewcommand{\arraystretch}{3}
    \begin{tabular}{cccc}
        \multirow{2}[2]{*}[2mm]{
                \shortstack{\includegraphics[width=4cm]{./images/result/pasta/000_gt.png} 
                \\ Fern}} 
        & \begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/space023/crop1/org.png}\end{subfigure}
        & \begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/space023/crop1/our.png}\end{subfigure}
        & \begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/space023/crop1/deepv.png}\end{subfigure} 
        \bigstrut \\
        & \begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/space023/crop2/org.png}\end{subfigure}
        & \begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/space023/crop2/our.png}\end{subfigure}
        & \begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/space023/crop2/deepv.png}\end{subfigure} 
        \bigstrut \\
        
        \multirow{2}[2]{*}[2mm]{
                \shortstack{\includegraphics[width=4cm]{./images/result/space023/ground_truth_06.png} 
                \\ Orchids}} 
        & \begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/space023/crop1/org.png}\end{subfigure}
        & \begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/space023/crop1/our.png}\end{subfigure}
        & \begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/space023/crop1/deepv.png}\end{subfigure} 
        \bigstrut \\
        & \begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/space023/crop2/org.png}\end{subfigure}
        & \begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/space023/crop2/our.png}\end{subfigure}
        & \begin{subfigure}[b]{0.10\textwidth}\includegraphics[width=\textwidth]{./images/result/space023/crop2/deepv.png}\end{subfigure} 
        \bigstrut \\

    \end{tabular}
    \caption{Comparisons on test-set views of NeRF's real forward-facing dataset.
    NeRF has more complete geometry than LLFF, as shown in Orchid's petals. 
    In the other hand, LLFF is better in very fine detail texture, as shown in Leaves' crop.
    Our method is able to well represent both fine detail and geometry. 
    }
\end{figure*}

==> content/RecycleBin/UNUSED__3method.tex <==
\section{Approach}
Given a set of images taken from multiple views of a scene, our goal is to construct a 3D representation that can render novel views with view-dependent effects \emph{in real-time}. To solve this problem, we employ a representation similar to multiplane image \cite{zhou2018stereo} but with significant improvements, which include a novel view-dependent pixel representation that can handle non-Lambertian surfaces, a hybrid implicit-explicit parameter modeling to improve fine details, and a method for learning such a representation. Our approach focuses on forward-facing captures with around 12 images or more, such as those taken casually by a smartphone in front of a scene. In the following sections, we first briefly review the original MPI representation, then explain our novel representation and a learning method for inferring it.
%we consider the scene reconstruct problem using MPI. %E1 "consider the scene reconstruct" WC
%we can use the standard Structure-from-Motion algorithm to estimates the required intrinsics and extrinsics from them.
%These calibrated photos can come from unstructured captures that are processed using any standard Structure-from-Motion algorithm that estimates the required intrinsics and extrinsics. %E1 "hand-held capture" already said this>
%(from LLFF) The overall strategy of our method is to use a deep learning pipeline to promote each sampled view to 
%Our final goal is to find a scene representation that can realistically render novel views between our set of input views.
%The resulting geometry and reflection need to allow rendering in realtime using a standard computer. 
%In the following sections, we first briefly review the original MPI representation, then explain our proposed MPI model and the method for inferring MPIs.
%E1 "to be able to rendered" "then describe our proposed method for inferring MPIs "

\begin{figure}
  \includegraphics[scale=0.16]{./images/mpi_pipeline.png}
  \caption{The overview of the model architecture. We reconstruct an MPI by sampling pixel's position $x,y$ and plane depth $d$ and taking to an MLP as inputs to output alpha and view-dependent coefficients, then combining them with an explicit MPI of the constant term to create RGB$\alpha$ MPI. The resulting image is the product of the composite operation over MPI. We use a gradient-based optimization to jointly train weights of MLP and the explicit MPI by comparing it with the original photo. 
  }
  \label{fig:overview}
\end{figure}

\subsection{Original MPI Representation}
Multiplane image \cite{zhou2018stereo} is a 3D scene representation that consists of a collection of $D$ planar images, each with dimension $H\times W\times 4$ where the last dimension contains RGB values and alpha transparency values. These planes are scaled and placed equidistantly either in the depth space (for bounded close-up objects) or inverse depth space (for scenes that extend out to infinity) along a reference viewing frustum (see Figure \ref{fig:overview}). 
%In this work, the depths of these planes are manually specified to roughly cover the content of the scene by first setting the maximum and minimum depth planes. Each inner plane is then placed . %E1 traditionally last channel



Rendering an RGB$\alpha$ MPI in any target view can be done by first warping all its planes to the target view via a homography that relates the reference and target view and apply the composite operator \cite{Porter1984Comp}. In particular, let $c_i\in \mathbb{R}^{H\times W \times 3}$ and $\alpha_i\in \mathbb{R}^{H\times W \times 1}$ be the RGB and alpha ``images'' of the $i^\text{th}$ plane respectively, ordered from back to front. And denote $A=\{\alpha_1,\alpha_2,...,\alpha_D\}$, $C=\{c_1,c_2,...,c_D\}$ as the sets of these images. This MPI can then be rendered in a new view, $\hat{I}$, using the composite operator $O$:
\begin{equation}\label{eq:1}
    \hat{I} = O(W(A),W(C))
\end{equation}
where $W$ is a homography warping function that warps each image to the target view, and $O$ has the form:
\begin{equation}
    O(A,C) = \sum^{D}_{d=1}c_d T_d(A), \;  T_d(A) = \alpha_d \prod^{D}_{i=d+1} (1-\alpha_i)
\end{equation}
This rendering equation is completely differentiable, thus allowing MPI to be inferred through image reconstruction loss \cite{zhou2018stereo,flynn2019deepview}.

\subsection{View-Dependent Pixel Representation}
One main limitation of MPI is that it can only model diffuse or Lambertian surfaces, whose colors appear constant regardless of the viewing angle.\footnote{A single MPI can simulate planar reflections to some extent by placing the reflected content on one of its planes \cite{flynn2019deepview}.} In real-world scenes, many objects are non-Lambertian such as a ceramic plate, a glass table, or a metal wrench. These objects exhibit view-dependent effects such as reflection and refraction (e.g. in Figure \ref{fig:viewdept-phenomenon}). Reconstructing these objects with MPI not only makes the objects appear unrealistically dull without reflections, but can also lead to errors in the reconstructed geometry as shown in Figure \ref{fig:noviewdep}. This is because the brightness constancy assumption, which is a basis for image matching invariant and 3D reconstruction, is violated. 

To allow for view-dependent modeling without relying on multiple MPIs (e.g. in \cite{mildenhall2019local}), we modify the pixel color representation in MPI, originally stored as RGB values, by parameterizing each color value as a function of the viewing direction $\mathbf{v}=(v_x, v_y, v_z)$. This results in a 3-dimensional mapping function $c(\mathbf{v}): \mathbb{R}^3 \rightarrow \mathbb{R}^3$ for every pixel. However, storing this explicitly is prohibitive and not generalizable to unobserved angles. Regressing the color directly from $\mathbf{v}$ (and the pixel location) with a neural network, as is done in e.g. \cite{mildenhall2020nerf}, is possible though inefficient for real-time rendering. Our key idea is to approximate this function with a linear combination of \emph{learnable} basis functions $\{H_l(\mathbf{v}): \mathbb{R}^3 \rightarrow \mathbb{R}\}$ over the spherical domain described by vector $\mathbf{v}$:

%Not only do the view-dependent effects of these objects 
%E1 "view-dependent" is adj
%The view-dependent effect is a natural phenomenon that caused by a property of a material that interacts with light. For example, the reflection and the refraction (See Figure \ref{fig:viewdept-phenomenon}). %E1 "reflection and refraction" is not properties of light
%The standard static MPI alone can't well represent the view-dependent effects.%t like shadow or specular highlights. 
%We need our color channel in MPI to rely on the direction toward the virtual camera.
%Assuming that we want the color $c$ in each pixel be a function of a unit vector $\mathbf{v}=(v_x, v_y, v_z)$ which represent the viewing direction,
%we would like to approximate the function with a linear combination of basis function $\{H_l(\mathbf{v})\}$ over the vector $v$. i.e. %E1 "over the view direction"
\begin{equation} \label{eq:basis}
     c(\mathbf{v}) =  k_0+\sum^{N}_{n=1} k_n H_n(\mathbf{v}) % = k_0 + \vec{k} \cdot \vec{H}(v)
\end{equation}
where $k_n \in \mathbb{R}^3$ are RGB coefficients or reflectance parameters of $N$ basis functions. In general, there are several ways to define a suitable set of basis functions. Spherical harmonics basis is one common choice used heavily in computer graphics to model complex reflectance properties \cite{sh}. Fourier's basis or Taylor's basis can also be used. However, one shortcoming of these ``fixed'' basis functions is that in order to capture high-frequency changes within a narrow viewing angle, such as sharp specular highlights, the number of basis required can be very high. This in turns requires more reflectance parameters which make both learning these parameters and rendering more difficult.

With learnable basis functions, our modified MPI outperforms other versions with alternative basis functions that use the same number of coefficients in experiment \ref{PSNRvs}, and produces convincing results on numerous challenging surfaces such as silverware and CDs \ref{cdfig} --- all in real-time.

To summarize, our modified MPI contains the following parameters per pixel: $\alpha, k_0, k_1, \ldots, k_N$; and global basis functions $H_1, H_2,\dots, H_N$ shared across all pixels.

%In our final model, each pixel consists of $N+1$ basis coefficients, i.e., $k_0,...,k_N \in \mathbb{R}^3$, and the original alpha weight.
%%% move to experiment sec
%As a simple example, 2nd order spearical harmonics basis defined as:
%$$\vec{H}(\mathbf{v}) = [v_x, v_y, v_z, v_x v_y, v_y v_z, 3v_z^2-1, v_x v_z, v_x^2-v_y^2] .$$
%Spherical harmonics has orthogonal property and well approximate function in surface sphere domain.
%Fourier's basis or Taylor's basis can also be used too.

%In conclusion, each pixel in our MPI doesn't directly contain color $c$ value, but our MPI consists of $N+1$ basis coefficients of view-dependent color $k_0,...,k_N$ and along with an alpha weight $\alpha$. %E1 "doesn't contain color c" it does

%The computation  is simple by considering the linear combination term as a dot product: %E1 "can also be consider " WC
%\begin{equation} \label{vec_form}
%    c(\mathbf{v}) = k_0 + \vec{k} \vec{H}^\top(v)
%\end{equation}
%where $ \vec{k} = [k_1,..., k_N]$ and $ \vec{H}(v) = [H_1(v),...,H_N(v)]$.
%Note that we call the first coefficient or the constant term $k_0$ as base color.
%The performance of expression is limited by the number of basis functions $N$. When $N$ gets larger, may lead to a storage problem. %E1 "the performance ..." is not sentence
%We define $\vec{H}'(v)=g(\vec{H}(v))$ where $g:\mathbb{R}^N \rightarrow \mathbb{R}^n$ is a small learnable neural network.
%Replacing $H(v)$ with $H'(v)$ in (\ref{vec_form}) can transform function to a new coordinate system such that the number of dimensions is reduced 
%without sacrificing result quality.


\begin{figure}
    \label{light field}
       \centering
     \begin{subfigure}[b]{0.22\textwidth}
         \centering
         \includegraphics[width=\textwidth]{./images/view1.png}
         \caption{$1^{st} view$}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.22\textwidth}
         \centering
         \includegraphics[width=\textwidth]{./images/view2.png}
         \caption{$2^{nd} view$}
         \label{fig:three sin x}
     \end{subfigure}
  \caption{An illustration of the light field at different viewing angles. The standard RGB$\alpha$ MPI can't handle the reflection on the metal or the refraction on the lens.
  %With our light field estimation, our results clearly depict not only reflection  on stainless pipe but also refraction in len.
        }
  \label{fig:viewdept-phenomenon}
\end{figure}



\subsection{Modeling MPI with Neural Networks} %change to traing stratigy
Given our modified MPI and the differentiable rendering equation \ref{eq:1}, one can directly optimize for its parameters that best reproduce the training views. However, as demonstrated in earlier work \cite{flynn2019deepview}, doing so would lead to a noisy MPI result that overfits the training views and fails to generalize. Inspired by recent work of Deep Image Prior \cite{ulyanov2018deep} and NeRF \cite{ulyanov2018deep}, we solve this problem by regressing these parameters with multilayer perceptrons (MLPs) from spatial conditioning, i.e., pixel coordinates. In particular, we use two separate MLPs; one for predicting per-pixel parameters given the pixel location, and the other for predicting all global basis functions given the viewing angle. The motivation for using the second network is to ensure that the prediction of the basis functions, which are global, is independent of any particular pixel location.

%One could try to use standard image denoising prior such as total variation,
%but this prior still seems insufficient and produces unsatisfactory results for challenging regions. 

%We're inspired by Deep Image Prior \cite{ulyanov2018deep} and NeRF \cite{ulyanov2018deep}. %E1 
%We use an MLP as a deep prior on MPI.
%We call this as Deep Multiplane Image Prior.
Our first MLP is modeled as $F_\theta$ with parameter $\theta$:
%Each pixel in our MPI has a spatial location and depth $\mathbf{x}=(x,y,d)$.
%The MLP is modeled as $F_\theta$ with parameter $\theta$:
\begin{equation}
    F_\theta: (\mathbf{x}) \rightarrow (\alpha, k_1, k_2,...,k_N)
\end{equation}
where $\mathbf{x}=(x,y,d)$ contains the location information of pixel $(x, y)$ at plane $d$. Note that $k_0$ is not predicted by $F_\theta$ but will be stored explicitly in our implicit-explicit learning strategy, which will be explained in the upcoming section. The second network is modeled as $G_\phi$ with parameter $\phi$:
\begin{equation}
    G_\phi: (\mathbf{v}) \rightarrow (H_1, H_2, ..., H_N)
\end{equation}
where $\mathbf{v}$ is the normalized viewing direction. 

It is interesting to note that unlike other networks used in other MPI learning techniques, our networks do not take as input any information from the training images but will receive supervision from those images through an image reconstruction loss. This kind of parameter estimation and other coordinate regressions (e.g., \cite{park2019deepsdf, mildenhall2020nerf}) can be thought of as applying a deep image prior \cite{ulyanov2018deep} on the estimated parameters. In other words, instead of allowing the estimated parameters to take arbitrary values which are prone to overfitting, we regularize these parameters by only allowing them to take on certain values that are in the span of a deep neural network's output. When the network is convolutional, the span of the network can capture the natural image manifold surprisingly well \cite{ulyanov2018deep}. In our case, we found that deep priors based on multilayer perceptrons can regularize our MPI and produce superior results compared to a direct optimization without the deep priors or with a standard regularizer such as total variation.  

%Surprisingly, the span of a network such as convolutional neural network can capture a natural image manifold.
%All unknown parameters in our MPI can then be inferred by optimizing these two networks. 
%Once these two networks are optimized, 
\subsection{Implicit-Explicit Learning Strategy} 
One observation when modeling $k_n$ (or ``coefficient texture'' when $k_n(x, y)$ is evaluated on all pixels) with an MLP is that the network has difficulty reproducing the high-frequency content of the texture (similar reports in \cite{sitzmann2020implicit,mildenhall2020nerf,tancik2020fourier}). The high-frequency content in our textures does not necessarily come from parts of the scene with complex geometry, but it can come from a simple geometry with detailed texture, such as the graphics of Tony the Tiger on a cereal box. We found that simply storing the base color $k_0$ explicitly helps ease the burden of compressing and reproducing details in these textures and allows the network to converge faster, and more importantly, produce sharper results. Thus, we employ this implicit-explicit learning strategy and use MLPs to predict every parameter except $k_0$ which will be optimized explicitly.

\textbf{Coefficient Sharing:} In practice, computing and storing all $N+1$ coefficients for all pixels for all $D$ planes can be expensive for both training and rendering. In our experiment, we use a coefficient sharing scheme where every $M$ planes will share the same coefficients, but not the alphas. That is, each plane still has its own alpha image, but there is a single set of $\{k_0, ..., k_N\}$ for planes $1$ to $M$, and another set for planes $M+1$ to $2M$, and so forth. With proper $N$ and $M>1$, we do not observe any significant degradation in the visual quality, but a significant gain in speed and compactness.


%Since storing $k_0$ explicitly for all $D$ planes can be expensive for large, dense MPI, in our experiment, we can reduce the number of $k_0$ images by sharing them across multiple layers. In particular, 

%Talks about $k_0$ being explicit and layers sharing.
%To infer our MPI, we optimize the parameter $\theta$ and $\phi$ 
%to represent components in our MPI. %
%Instead of representing every component with implicit function, 
%we found that keeping the first coefficient $k_0$ (or the constant term of the expansion) as an explicit structure in MPI help model obtain result faster. %E1 need to proporty define "explicit"

Finally, to optimize our model, we evaluate the two MLPs to obtain the implicit parameters, render an output image, and compare it to the ground-truth image from the same view. We use $L_2$ image reconstruction loss and a total variation on $k_0(x, y)$ as our minimization objective. Our approach is summarized in Algorithm 1.
%from a training view using Equation \ref{eq:1}
%We compare the rendered images with the ground truth images. %, named it reconstruction loss. %E1 "name it"
%We minimize the reconstruction loss alongside a total variation loss of 0th order coefficient $K_0$ to optimize network parameter $\theta$.






\begin{algorithm}
\SetAlgoLined
 initialize: $\theta, \phi, K_0$\;
 pre-compute $\mathcal{X}$ pixel coordinate for each pixel\; %E1 ?
 \For{Iteration=0 to maxIter}{
    sampling image $I_i$\;
    compute viewing direction $\mathcal{V}_i$ by
    $
    \begin{matrix}
       \mathcal{V}_i = \mathcal{X}- \text{center of projection of} \:I_i \\
       \mathcal{V}_i = \mathcal{V}_i / \| \mathcal{V}_i \|
    \end{matrix}$
    \;
    compute $ (A,\vec{K}) = F_\theta(\mathcal{X})  $ where $\vec{K} = [K_1, K_2,...,K_N] $\;
    compute view-dependent color $ C = K_0 + \vec{K} \cdot \vec{H}(\mathcal{V}_i)$\;
    compute rendered image $\hat{I}_i = O(W_i(A),W_i(C)) $ \;
    compute loss function by  $ L = \| \hat{I}_i-I_i \|^2 +\gamma \text{TV}(K_0) $ \;
    update $\theta, K_0$ with ADAM$(\nabla_{\theta,K_0}L)$ \;
    }
   \KwResult{$A,K_0,K_1,...,K_N$} 
 \caption{MPI training algorithm}
\end{algorithm}
%at inferent time every thing is convert into MPI wih

%Each one consists of a color $c=(r,g,b)$ and alpha weight $\alpha$.
%In NeRF this problem can be formulate by $F_\theta (\mathbf{x},\mathbf{v})=(\alpha, c)$. 
%However, this evaluation take a long time to calculate and can't be use in real-time render.


\subsection{Real-time Rendering} 
Every model parameter in our MPI can be converted to an image in a straightforward way. For example, we can evaluate $F_\theta$ on all pixel coordinates and $G_\phi$ on some pre-defined viewing span. Given these pre-computed images, we can implement Equation \ref{eq:1} in a fragment shader in OpenGL/WebGL and acheive a real-time view-dependent visualization of our captured scene.

==> content/RecycleBin/experiment_network_structure.tex <==
\subsubsection{Network architectures} %May move to sup mat
There is a vast body of work dedicated to find the best network for represent 3d scene. NeRF\cite{mildenhall2020nerf} use a ReLU network with positional encoding (PE) which help network learn higher frequency function. Latter NeRf's team have another work \cite{tancik2020fourier} replace the positional encoding with Fourier feature mapping and show that it can out perform the previous. SIREN\cite{sitzmann2020implicit} concurrently introduced another way to represent by using a sine function as the activation function all layers in the network. This allows the network to learn high frequency without any input mapping.
We simplify all above design by remove all the concatenation connection. We use 6 fully-connected layers, each with 256 channels. 
The result is shown in Table \ref{architecture}. The SIREN network not only use lower number of parameters in the fist fully-connected layer but also have best in every score. However, the winning gap is not large.

\begin{table}%
\caption{Comparing Network architecture choices}
\label{architecture}
\begin{minipage}{\columnwidth}
\begin{center}
\begin{tabular}{llll}
  \toprule
  Method                                     & PSNR    & SSIM    & LPIPS\\ 
  ReLU Net. with PE.             & 27.38    & 0.961    & 0.1200\\
  ReLU Net. wtih FF              & 27.43    & 0.962    & 0.1190\\
  SIREN                          & 27.56    & 0.964    & 0.1142\\
  Skip Net.                      & 27.52    & 0.964    & 0.1146\\
  \bottomrule
\end{tabular}
\end{center}
\bigskip\centering

\end{minipage}
\end{table}%



% \subsection{Ablation studies} % this one is about Network sturecure
% In this subsection, we study our network design decisions that affect the quality of rendered images.  This experiment run on 4 scenes which is scene063 from Deepview's space dataset, flower, trex and room scene from NeRF's dataset.
% We divide the experiment into two parts. In the first part, we vary the number of MLP layers and number of hidden node in each layers.
% The best performance model is the architecture that contain 6 layers of MLP and each layer contain 256 nodes.

% In this experiment we validate our algorithm with an ablation study in Table \ref{tab3}.
% The first row show a complete version of our model.
% In second row, we shows a minimalist version of our model without MLP which % corresponds to just the directly optimized an MPI with SGD.
% The performance is bad as expected.
%In the third row, we only remove positional encoding from the network. From our experiment, we see that the boundary of objects is blurred.
%In forth row, we remove coordinates with high frequency mapping to quantitative performance of them. The results are better in terms of sharp boundary than not using positional encoding at all.
%In fifth row, we input high frequency positional encoding abundantly (32 levels and 16 levels).
%In the last row, we show the effect of reducing number of input images. Our algorithm have a hard time to place object in the right plane.

%We validate our algorithm’s design choices and parameters with an extensive ablation study in Table 2.
% We present results on one of our synthetic scenes with complex geometry and non-Lambertian materials (Lego).
% Row 9 shows our complete model as a point of reference. 
%Row 1 shows a minimalist version of our model without positional encoding (PE), view-dependence (VD), or hierarchical sampling (H).
%In rows 2–4 we remove these three components one at a time from the full model,
%observing that positional encoding provides the largest quantitative benefit of these three contributions (row 2),
% followed by view-dependence (row 3), and then hierarchical sampling (row 4).
% Rows 5–6 show how our performance decreases as the number of input images is reduced.
%Note that our method’s performance using only 25 input images still exceeds NV, SRN, and LLFF across all metrics when they are provided with 100 images
%In rows 7–8 we validate our choice of the maximum frequency L used in our positional encoding for x
%(the maximum frequency used for d is scaled proportionally).
% Only using 5 frequencies reduces performance, but increasing the number of frequencies from 10 to 15 does not improve performance.
%We believe the benefit of increasing L is limited once 2L exceeds the maximum frequency present in the sampled input images (roughly 1024 in our data).

%\begin{table}%
%\caption{An ablation study of our model on TREX from Nerf dataset %\cite{mildenhall2020nerf}.}
%\label{tab3}
%\begin{minipage}{\columnwidth}
%\begin{center}
%\begin{tabular}{lll}
%  \toprule
%                            & PSNR  & SSIM  \\ \midrule
%  Complete Model            & 25.6110  & 0.9119  \\
%  No MLP (direct opt MPI)       & 30.8834 & 0.9549 \\
%  No Frequency transform     & 22.4949  & 0.8682\\
%  Low frequency transform       & 23.8289 & 0.8930\\
%  High frequency transform      & 23.6663 & 0.8938 \\
%  Fewer input image             &         & \\
%  \bottomrule
%\end{tabular}
%\end{center}
%\bigskip\centering
%\footnotesize\emph{Source:} This is a table
% sourcenote. This is a table sourcenote. This is a table
% sourcenote.

 %\emph{Note:} This is a table footnote.
%\end{minipage}
%\end{table}%

%\begin{table}%
%\caption{An ablation study of network architecture on Flower, Room, Trex from %Nerf dataset \cite{mildenhall2020nerf}.}
%\label{tab3}
%\begin{minipage}{\columnwidth}
%\begin{center}
%\begin{tabular}{lll}
%  \toprule
%                            & PSNR  & SSIM  \\ \midrule
%  128 hidden nodes & 21.6290 & 0.8944 \\
%  256 hidden nodes & 21.6858      &0.8976\\
%  5 layers      & 21.6290  & 0.8944\\
%  6 layers      & 21.8438 & 0.8973\\
%  7 layers      & 21.6956 & 0.8933 \\
%  8 layers      & 21.5055 & 0.8927 \\

%  \bottomrule
%\end{tabular}
%\end{center}
%\bigskip\centering
%\footnotesize\emph{Source:} This is a table
% sourcenote. This is a table sourcenote. This is a table
% sourcenote.

 %\emph{Note:} This is a table footnote.
%\end{minipage}
%\end{table}%


==> content/RecycleBin/note.tex <==
%While NeRF\cite{mildenhall2020nerf} uses an implicit function for both RGB and alpha, there is an explicit representation which also commonly used. 
%However, explicit MPI demands a regularizer like the total variation in order to solve an under-constrained problem. 
In this experiment, we validate our design decision that stores base color $K_0$ explicitly while modeling other parameters with implicit functions. Additionally, in Table \ref{tab:represent} we explore all 8 alternatives for representing alpha ($A$), base color ($K_0$), and view-dependent coefficients ($K_1,...,K_N$), ranging from a fully implicit model (Im-Im-Im) to a fully explicit model (Ex-Ex-Ex). Note that the fully explicit model corresponds to optimizing the rendering equation directly without any deep priors on the parameters. 
The result shows that our Im-Ex-Im outperforms other alternatives and storing base color $K_0$ explicitly is beneficial also to other configurations regardless of the modeling choices for the alpha and coefficients. Qualitatively, our method produces significantly better detail compared to the fully implicit model and cleaner results that generalize better than the fully explicit model (please see our supplementary).
%by studying how the implicit function and explicit structure form affect the quality of each model component. 
%Before, we select the best combination for our representation

 %shows a comparison selects two approaches: a neural implicit function and an explicit MPI structure, in representing alpha ($A$), base RGB color ($K_0$), and view dependent effect ($K_1,...,K_N$). PSNR, SSIM and LPIPS are provided for each of the 8 combinations. 
 %As we can see, alpha weights represented by an implicit function is clearly beneficial for all of the cases. 
%We suspect that the reason is from the nature of the alpha which is mostly continuous in space. By contrast, base RGB color using an explicit representation is better in every cases. Probably because explicitly modeling is easier for the model to converge to high frequency. 

%%% Talk about optimization
% - explicit mpi: noisey, transparent
% - implicit: blurry
% - we use hybrid
Estimating a standard explicit MPI requires solving each value in pixels on each plane, resulting in a huge number of unknown variables. 
Similar to many other inverse problems, this problem is under-constrained. 
The basic implementation of solely optimizing the unknowns given observations would yield an over-fitted solution where the rendering only looks good from the angles it's seen before during training.
Even optimizing MPI with traditional regularization like total-variation, the obtained results are still noisy and transparent because of ambiguity of an explicit MPI itself.
Another way of handling this issues is using the concept of implicit prior.
We can represent each pixel value in our MPI as the output of a multilayer perceptron (MLP) and optimize the MLP parameters.
This can reduce the number of parameters that need to be optimized as well as the number of possible solutions.
This can also be considered as neural scene representations similar to DeepSDF \cite{park2019deepsdf} and NeRF \cite{mildenhall2020nerf}.
However, the limited network capacity in these approaches often gives blurry results.
Also complexity of evaluation a neural network in training process is time-consuming.
Instead of modeling the entire MPI with an explicit MPI or implicit neural network.
We found that keeping some variables that need high resolution in an explicit form is easier for our model to reconstruct the scene.
We combine the power of deep prior by neural implicit fields, with explicit MPI base structure to create a hybrid approach to optimize an MPI.


Estimating an MPI explicitly would yield an over-fitted solution where the obtained results are noisy and transparent because of ambiguity of an explicit MPI itself.
Another way of estimating is by using the concept of implicit deep prior.
We can represent each pixel value in our MPI as the output of a multilayer perceptron (MLP) and optimize the MLP parameters.
This can also be considered as neural scene representations similar to DeepSDF \cite{park2019deepsdf} and NeRF \cite{mildenhall2020nerf}.
However, the limited network capacity in these approaches often gives blurry results.
Instead of modeling the entire MPI with an explicit MPI or implicit neural network.
We found that keeping some variables that need high resolution in an explicit form is easier for our model to reconstruct the scene.
We combine the power of deep prior by neural implicit fields, with explicit MPI base structure to create a hybrid approach to optimize an MPI.


An implementation of our model requires a prohibitive amount of ...
In the absence of a strong prior





A. Additional Implementation Settings






A.1. Data Preparation Details

Accurate camera poses and intrinsic parameters are very important for  our  calculation.
After we capture a scene, e need to preprocess the scene.
We use an open-source software package named COLMAP [3].
The software runs Struction-from-Motion (SfM) algorithm and solves distortion parameters, 
which takes a few moments for a set of input images.
We calibrated not only our captured scenes but also scenes from NeRF’s dataset.



A.2. Data sampling

In the training process,
we first randomly select an image from a training set in a selected scene.
We then randomly select 2666 pixel locations.
For any selected pixel location(x, y), 
we render the pixel(x, y), (x, y+ 1) and (x+ 1, y).
We use 3 computed pixel values to evaluate image gradient,
which used to compare with the original image by reconstruction loss


%%% Data preparation Details
% 1 radoa; distortion, and config used



%%% Data Sampling
For each scene, we train our model with 4,000 epochs.
In each epoch, we loops over set of training image.
In each image, we randomly select 2667 pixel locations.
For any selected pixel location $(x, y)$, 
we render the pixel $(x, y)$, $(x, y+1)$ and $(x+1, y)$.
We use 3 computed pixel values to evaluate image gradient,
which used to compare with the original image by reconstruction loss $L_{\test{rec}}$.

We run inference every 200 epochs.
%we evaluate all pixel in the testing image.
For evaluation, we use 3 evaluation matrics including
PSNR and SSIM from scikit-image software package and VGG variant of LPIPS as implemented in https://github.com/richzhang/PerceptualSimilarity.


We implement our model with PyTorch.
We also use DistributedDataParallel (DDP) which supports multi-GPU training and inference.
However, only MLP for $F_\theta$ and $G_\phi$ got benefit from multi-GPU.
For 192 layers MPI, the model need to evaluate each MLP 192 coordinates per 1 pixel.
For multi-GPU, all 192 coordinates are split to GPUs and transfer back to 1 GPU.


==> content/supplyment2.tex <==


\section{Implementation Details}
%We optimize MPIs both texture and structure of 3D objects using a sparse set of (10-20)inputs together with its cameras' intrinsic and extrinsic from Deepview and NeRF.
In our work, to prevent MPIs breaking, the number of layers and sublayers for MPIs are 20 and 15, respectively, 300 planes combining together. For network structure (see \figref{tab2} for overall graphic), we use a 4 fully connected layers to obtain alpha and information related specular reflection. To alleviate the issue that gradient got stuck at near planes because of low net transmittance and MPIs doesn't learnt anything, we set a 5 offset bias to the channel producing alpha throughout the training process.

For the specular model, 7 outputs from MLP are needed. We use three outputs to represent normal surface, 1 for shininess of surfaces and the final three channels for specular constant. To eliminate numerical issue, the maximum of shininess is set to 30 instead of unbounded value. Ten light directions and their intensities are optimized.


%Direct optimization on all RGB planes is often resulted in poor visual quality due to under constrained solutions. 
Reducing Memory at training time is challenging. We need to our method can be back-propagate the gradients.
Memory issue is our mainly the problem to generate realistic and high resolution view synthesis. 
Therefore, we introduced sampling ray across all planes. The amount of memory that is reduced depends on the numbers of ray sampled. Instead of random sampling, we choose L-shaped mini rays sampling. We do this on the purpose of getting rid of high frequency artifacts from positional encoding. These artifacts occur often at texture-less area. With the L-shaped rays, image gradient are computed on 2x1 or 1x2 grid. From the observation, applying image gradient loss on this grid leads to dusty spaces where there are a lot of texture. We computed this loss only on area where image gradient is lower than 0.005. 
 
Sampling ray instead of training all rays in the rendered view reduces MLP's capacity because network forgot what it had learnt and less sampling areas resulted in less details and missing thin structures. To increase rays, we trained parallel on multiple GPUs.In our experiments, we use up to 12000 rays on 1 NVIDIA 2080Ti and can go up to 48000 on 4 GPUs. During optimization, we pick Adam optimizer with learning rate started at 0.01 and decayed rate at 0.5 for every 10000 steps until it converges at 100000 steps (about 8 hours). (SUPPLEMENT) Inspired by stochastic sampling for Nerf, we trained MLP with stochastic planes positions allowing us to up-sample the alpha planes during inference up to 4 times. In our experiments, we trained 72 planes stochastically and get up to 288 planes. 

%We use the Adam optimizer with learning rate up to 0.1.
%Taking huge learning rate requiring only a few iterations at inference time.
%The optimization took around 1k - 4k iterations to converge on a single scene.

  
\begin{figure}
  \label{network}
  \includegraphics[scale=0.42]{./images/network.PNG}
  \caption{The neural network structure that has been used in our experiments. Each boxes represent node vectors and arrows represent operations. Every fully connected layers used LReLU activation (Leaky Rectified Linear Activation), except the last one which use sigmoid activation.}
  \label{fig:one}
\end{figure}


\begin{table}%
\caption{PSNR.}
\label{tab3}
\begin{minipage}{\columnwidth}
\begin{center}
\begin{tabular}{lllll}
  \toprule
                    & SRN  & LLFF & NeRF  & Our   \\ \midrule
  Fortress      & 26.63 & 29.40 & 31.16 & \textbf{31.62} \\
  Fern          & 21.37 & 22.85 & 25.17 & \textbf{25.42} \\
  Flower        & 24.63 & 25.46 & 27.40 & \textbf{28.74} \\
  T-rex         & 22.87 & 24.15 & 26.80 & \textbf{28.12} \\
  Leaves        & 18.24 & 19.52 & 20.92 & \textbf{21.90} \\
  Horns         & 24.33 & 24.70 & 27.45 & \textbf{27.93} \\ 
  Orchids       & 17.37 & 18.52 & 20.36 & \textbf{20.46} \\
  Room          & 27.29 & 28.42 & \textbf{32.70} & 32.00 \\
  \midrule
  \bottomrule
\end{tabular}
\end{center}
\bigskip\centering
\end{minipage}
\end{table}%

\begin{table}%
\caption{SSIM.}
\label{tab3}
\begin{minipage}{\columnwidth}
\begin{center}
\begin{tabular}{lllll}
  \toprule
                    & SRN  & LLFF & NeRF  & Our   \\ \midrule
  Fortress      & 0.641 & 0.872 & 0.881 & \textbf{0.951} \\
  Fern          & 0.611 & 0.753 & 0.792 & \textbf{0.940} \\
  Flower        & 0.738 & 0.844 & 0.827 & \textbf{0.930} \\
  T-rex         & 0.761 & 0.857 & 0.880 & \textbf{0.947} \\
  Leaves        & 0.520 & 0.697 & 0.690 & \textbf{0.830} \\
  Horns         & 0.742 & 0.840 & 0.828 & \textbf{0.927} \\
  Orchids       & 0.449 & 0.588 & 0.641 & \textbf{0.768} \\
  Room          & 0.883 & 0.932 & 0.948 & \textbf{0.972} \\
  \bottomrule
\end{tabular}
\end{center}
\bigskip\centering
\end{minipage}
\end{table}%

\begin{table}%
\caption{LPIPS.}
\label{tab3}
\begin{minipage}{\columnwidth}
\begin{center}
\begin{tabular}{lllll}
  \toprule
                    & SRN  & LLFF & NeRF  & Our   \\ \midrule
  Fortress      & 0.453 & 0.173 & 0.171 & \textbf{0.129} \\
  Fern          & 0.459 & 0.247 & 0.280 & \textbf{0.202} \\
  Flower        & 0.288 & 0.174 & 0.219 & \textbf{0.150} \\
  T-rex         & 0.298 & 0.222 & 0.249 & \textbf{0.196} \\
  Leaves        & 0.440 & 0.216 & 0.316 & \textbf{0.168} \\
  Horns         & 0.376 & 0.193 & 0.268 & \textbf{0.183} \\
  Orchids       & 0.467 & 0.313 & 0.321 & \textbf{0.236} \\
  Room          & 0.240 & \textbf{0.155} & 0.178 & 0.164 \\
  \bottomrule
\end{tabular}
\end{center}
\bigskip\centering
\end{minipage}
\end{table}%

\subsubsection{Orthogonal Polynomials}
A set of polynomials $\{p_l(x)\}$ are said to be orthogonal over an interval $[a,b]$ if $p_l(x)$ is a polynomial of degree $l$, and for $m\neq n$
$$
\int^b_a w(x)p_n(x)p_m(x) dx = 0
$$
The most commonly used orthogonal polynomials are includes:
the Legendre polynomials that be given by
\[
L_n(x) = \sum^n_{i=1} {n\choose i}^2 \left(\frac{x-1}{2}\right)^i \left(\frac{x+1}{2}\right)^{n-i},
\]
and the Jacobi polynomials that be written as
\[
J_n(x) = \sum^n_{i=1} {n\choose n-i} {n+b \choose i} \left(\frac{x-1}{2}\right)^i \left(\frac{x+1}{2}\right)^{n-i}
\]
Note that, if $b=0$, then Jacobi polynomials become the Legendre polynomials.

$$
c(v) = \sum^n_{s=0} \sum^s_{l=-s} k_{ls} H^{(s)}_l(v)
$$
\subsubsection{Spherical Harmonics basis}
There is a standard way for constructing sphearical harmonics:
\begin{enumerate}
    \item choose the polynomials ${L_n(x)}$ which satisfy the orthogonality condition,
    \item define the adjoint function ${L_n^{(m)}(x)}$,
    \item construct the spherical harmonics by combination of $L_n^{(m)}(cos(\theta))$ wtih $\{\cos(m\phi), \sin(m\phi)\}$.
\end{enumerate}

Replacing the argument $x$ with $\cos \theta$, we get a set of function $\{L_l^{(m)}(\cos\theta)\}$. Real valued SH functions are constructed from $L_l^{(m)}(\cos\theta)$ as:
\[
  Y^m_l(\phi,\theta) =
  \begin{cases}
    \cos(m\phi) L_l^{(m)}(\cos\theta) & \text{if $m>0$} \\
    \sin(-m\phi) L_l^{(-m)}(\cos\theta) & \text{if $m<0$} \\
    L^{(0)}_l(\cos\theta) & \text{if $m<0$}
  \end{cases}
\]

%\subsubsection{Hemi-shearical Harmonics basis}

%Shifted ALPs. using linear transformation of $x$ to $ax$ we get shifted ALPs over the interval $x\in[a,1]$:
The idea of hemi-shearical harmonics is restricting the spherical zone from $x\in[-1,1]$ to $x\in[0,1]$.
They're doing so by define shifted Legendre polynomials as
\[
\Tilde{L}^{(m)}_l (x) = L^{(m)}_l\left(2x - 1 \right)
\]

In the same sense that SH functions are constructed from Legendre polynomials, this basis functions $\{H^{(m)}_l(\phi,\theta)\}$ are constructed from shifted Legendre polynomials.
\[
  H^{(m)}_l(\phi,\theta) =
  \begin{cases}
    \cos(m\phi) \Tilde{L}_l^{(m)}(\cos\theta) & \text{if $m>0$} \\
    \sin(-m\phi) \Tilde{L}_l^{(-m)}(\cos\theta) & \text{if $m<0$} \\
    \Tilde{L}^{(0)}_l(\cos\theta) & \text{if $m=0$}
  \end{cases}
\]
In general we can shifted the polynomials to any domain $x\in[a,1]$ for $-1\leq a<1$ by.
\[
\Tilde{J}^{(m)}_l (x) = J^{(m)}_l\left(2\cdot\frac{x-1}{1-a} + 1 \right)
\]

Finally, we change the variable from $(\phi,\theta)$ to $v=(v_x,v_y,v_z)$ by the relation:
$$
v_x = \cos \phi \sin \theta, \quad v_y = \sin \phi \sin \theta, \quad v_z = \cos \theta.
$$
Some first few basis are:
\begin{align*}
H^{(0)}_0(v) &=1,  \\
H^{(-1)}_1(v) &=v_y \frac{b+2}{1-a}\sqrt{\frac{v_z-a}{v_z+1}}, \\
H^{(0)}_1(v) &=(v_z-1)\frac{b+2}{1-a}+1, \\
H^{(1)}_1(v) &=v_x \frac{b+2}{1-a}\sqrt{\frac{v_z-a}{v_z+1}}.
\end{align*}







